Well-tuned Simple Nets Excel on Tabular Datasets

Tabular datasets are the last "unconquered castle" for deep learning, with traditional ML methods like Gradient-Boosted Decision Trees still performing strongly even against recent specialized neural architectures. In this paper, we hypothesize that the key to boosting the performance of neural networks lies in rethinking the joint and simultaneous application of a large set of modern regularization techniques. As a result, we propose regularizing plain Multilayer Perceptron (MLP) networks by searching for the optimal combination/cocktail of 13 regularization techniques for each dataset using a joint optimization over the decision on which regularizers to apply and their subsidiary hyperparameters. We empirically assess the impact of these regularization cocktails for MLPs in a large-scale empirical study comprising 40 tabular datasets and demonstrate that (i) well-regularized plain MLPs significantly outperform recent state-of-the-art specialized neural network architectures, and (ii) they even outperform strong traditional ML methods, such as XGBoost.

==> Algorithms/bohb_algorithm.tex <==
\begin{algorithm}[h!]
\caption{BOHB}
\label{alg:bohb}
\begin{algorithmic}
    % \ttfamily
    \INPUT $b_{min}$, $b_{max}$ and $\eta$  
    \STATE \textbf{Initialization:} $s_{max}=\log_\eta \frac{b_{max}}{b_{min}}$
    \FOR{{\textit{s} in ($s_{max}$, $s_{max-1}$,...,0)}} 
    \STATE $n$ = $ \frac{s_{max} + 1}{s + 1}$ 
    \STATE Call SH routine with $\eta^{-s} \cdot b_{max}$
    \ENDFOR
    \OUTPUT \textit{Hyperparameter configuration with the smallest loss}
\end{algorithmic}
\end{algorithm}

==> Plots/baseline_violin_ranks.tex <==
\begin{figure}
    %\vspace{-0.5cm}
    \begin{center}
    {\includegraphics[width=0.5\textwidth]{Figures/baseline_violin_ranks.pdf}}
    \caption[Rank distribution for baselines and the regularization cocktail]{\textbf{Rank distribution for baselines and the regularization cocktail.} The rank distribution for each method is calculated on the test set over all datasets. Smaller is better.}
    \label{fig:benchmark_violin_ranks}
    \end{center}
    %\vspace{-0.1cm}
\end{figure}

==> Plots/baselines_test_error_comparison.tex <==
\begin{figure*}[tb]
    %
    \medskip
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=0.9\textwidth]{Figures/cocktail_vs_xgboost_error_rate.pdf}
      %\caption{Gain over the number of examples}
      %\label{fig:1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=0.9\textwidth]{Figures/cocktail_vs_autosklearn_error_rate.pdf}
      %\label{fig:2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=0.9\textwidth]{Figures/cocktail_vs_tabnet_error_rate.pdf}  
      %\caption{Gain over the test accuracy}
      %\label{fig:3}
    \end{subfigure}
    \caption[A summary of the gain that the full search spaced cocktail achieves compared state-of-the-art competitors.]{Comparison of our proposed dataset-specific cocktail against the state-of-the-art competitors. Each point represents a dataset and the gain is defined as the ratio of errors (error baseline / error cocktail) on the test set.} %Ak: No space, if we make a bit more space, we can uncomment. We illustrate the gain against the following competitors: XGBoost (left), autosklearn (middle) and TabNet (right).}
    \label{fig:cocktail_benchmarks_gain}
\end{figure*}

==> Plots/benchmark_cd_diagram.tex <==
\begin{figure}
    %\vspace{-0.3cm}
    \begin{center}
    {
    %\hspace*{-0.8cm}
    \includegraphics[width=0.6\textwidth]{Figures/benchmark_cd_diagram.pdf}}
    \caption[Benchmark Critical difference diagram]{\textbf{Critical difference diagram} generated with the Wilcoxon-Holm post-hoc analysis on 40 datasets. The diagram shows the ranks and the statistical significance of the results for every state-of-the-art competitor and our regularization cocktails.}
    \label{fig:benchmark_cd_diagram}
   \end{center}
\end{figure}


==> Plots/benchmarks_gain.tex <==
\begin{figure}[tb]
    %
    \medskip
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_xgboost_examples.pdf}
      %\caption{Gain over the number of examples}
      %\label{fig:1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_autosklearn_examples.pdf}
      %\label{fig:2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_tabnet_examples.pdf}  
      %\caption{Gain over the test accuracy}
      %\label{fig:3}
    \end{subfigure} \hfil
    \bigskip
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_xgboost_features.pdf}
      %\label{fig:4}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_autosklearn_features.pdf}
      
      %\label{fig:5}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=1.0\textwidth]{Figures/cocktail_improvement_tabnet_features.pdf}
      
      %\caption{Gain over the test accuracy}
      %\label{fig:6}
    \end{subfigure}
    \caption[A summary of the gain that the full search spaced cocktail achieves compared state-of-the-art competitors.]{Comparison of our proposed dataset-specific cocktail against the state-of-the-art competitors. Each point represents a dataset and the gain is defined as the ratio of errors (error baseline / error cocktail) on the test set.} %Ak: No space, if we make a bit more space, we can uncomment. We illustrate the gain against the following competitors: XGBoost (left), autosklearn (middle) and TabNet (right).}
    \label{fig:cocktail_benchmarks_gain}
\end{figure}

==> Plots/cd_diagram.tex <==
\begin{figure*}[ht]
    \begin{center}
    {\includegraphics[width=0.8\textwidth]{Figures/cd_diagram}}
    \caption[Critical difference diagram]{\textbf{Critical difference diagram} generated with the Wilcoxon-Holm post-hoc analysis on 40 datasets. The diagram shows the ranks and the statistical significance of the results for every individual regularization technique and our regularization cocktails.}
    \label{fig:cd_diagram}
    \end{center}
\end{figure*}

==> Plots/cocktail_gain_over_gb.tex <==
\begin{figure}[ht]
    \begin{center}
    {\includegraphics[width=\textwidth ]{Figures/gb_gain_dist.pdf}}
    \caption[Distribution of the gain of the regularization cocktail over gradient boosting]{\textbf{Distribution of the gain of the regularization cocktail over gradient boosting}. The gain is calculated as the test accuracy of the best hyperparameter configuration found by the regularization cocktail divided by the test accuracy of the best hyperparameter configuration found by the gradient boosting algorithm.}
    \label{fig:dist_cocktail_gain_over_db}
    \end{center}
\end{figure}



==> Plots/cocktail_gain_subsets.tex <==
\begin{figure}[ht]
    \begin{center}
    {\includegraphics[width=\textwidth ]{Figures/cocktail_gain_subsets.pdf}}
    \caption[Gain of the regularization cocktails]{\textbf{Gain of the regularization cocktails}. The gain of the best found regularization cocktails over the plain network is shown with the interrupted arrow lines.}
    \label{fig:gain_cocktail_subsets}
    \end{center}
\end{figure}



==> Plots/top3_result_summary.tex <==
\begin{figure}[t]
    \begin{center}
    {\includegraphics[width=\textwidth] {Figures/comparison_smaller_cocktail.pdf}}
    \caption[A summary of the gain that the full search-spaced cocktail achieves compared to the constrained one.]{\textbf{Gain of the full search space regularization cocktail} A summary of the gain that the full search space regularization cocktail achieves compared to the constrained version with only the top 3 methods. \textbf{From the left:} The gain on the test set over the number of examples, the gain over the number of features, and the gain over the test accuracy of the constrained version.}
    \label{fig:top3_summary}
    \end{center}
\end{figure}

%\noteml{Maybe we should plot the x-axis of the first two plots on a log-scale?}

==> Plots/top_3_summary_parts.tex <==
\begin{figure*}[htb]
    \centering %
    Our Dataset-specific vs. Top-5 Most Frequent (23 wins, 15 losses, 2 draws, $p$-value: 0.20446) \\
    \medskip
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=0.85\textwidth]{Figures/top5_freq_gain_examples.pdf}
      %\caption{Gain over the number of examples}
      %\label{fig:1}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth}
    
      \includegraphics[width=0.85\textwidth]{Figures/top5_freq_gain_features.pdf}
      %\label{fig:2}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=0.85\textwidth]{Figures/top5_freq_gain_accuracy.pdf}  
      %\caption{Gain over the test accuracy}
      %\label{fig:3}
    \end{subfigure}
    
    \medskip
    Our Dataset-specific vs. Top-5 Highest Ranks (30 wins, 9 losses, 1 draw, $p$-value: 0.00008) \\
    \medskip
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=0.85\textwidth]{Figures/top5_rank_gain_examples.pdf}
      %\label{fig:4}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=0.85\textwidth]{Figures/top5_rank_gain_features.pdf}
      
      %\label{fig:5}
    \end{subfigure}\hfil % <-- added
    \begin{subfigure}{0.33\textwidth} 
      \includegraphics[width=0.85\textwidth]{Figures/top5_rank_gain_accuracy.pdf}
      
      %\caption{Gain over the test accuracy}
      %\label{fig:6}
    \end{subfigure}
    \caption[A summary of the gain that the full search spaced cocktail achieves compared to the constrained one.]{Comparison of our proposed dataset-specific cocktail against the cocktail of the top-5 most frequent regularizers (top row), and the cocktail of the top-5 regularizers with the highest performance ranks (bottom row). Each point represents a dataset and the gain is defined as the ratio of errors (error baseline / error cocktail) on the test set. We illustrate the gain with three ablations: the number of data points (left), number of features (middle) and test accuracy (right).}
    \label{fig:top3_summary_v2}
\end{figure*}


==> Plots/traditional_diagram.tex <==
\begin{figure*}[ht]
    \begin{center}
    {\includegraphics[width=0.8\textwidth]{Figures/traditional_diagram.pdf}}
    \caption[Traditional algorithms critical difference diagram]{\textbf{Traditional algorithms critical difference diagram} generated with the Wilcoxon-Holm post-hoc analysis on 40 datasets. The diagram shows the ranks and the statistical significance calculated on the test set results for the different state-of-the-art models on tabular datasets and for our method. There are two versions of XGBoost in the diagram, where ES stands for Early Stopping. }
    \label{fig:traditional_diagram}
    \end{center}
\end{figure*}

==> Plots/violin_ranks_all_methods.tex <==
\begin{figure}[ht]
    \begin{center}
    \hspace*{-0.25cm}
    {\includegraphics[width=0.49\textwidth]{Figures/violin_ranks.pdf}}
    \caption[Rank distribution for the individual regularization methods and the regularization cocktail]{\textbf{Rank distribution for the individual regularization methods and the regularization cocktail.} The rank distribution for each method is calculated on the test set over all datasets.}
    \label{fig:violin_ranks_all}
    \end{center}
\end{figure}

==> Response/cocktail_vs_xgboost.tex <==
\begin{figure}[ht]
    \begin{center}
    {\includegraphics[width=0.2\textwidth]{Figures/cocktail_vs_xgboost_error_rate.pdf}}
    \label{fig:cocktail_vs_xgboost}
    \end{center}
\end{figure}

==> Response/early_stopping_comparison.tex <==
\begin{figure}[ht]
    \begin{center}
    {\includegraphics[width=0.45\textwidth]{Figures/early_stopping_data.pdf}}
    \label{fig:early_stopping_comparison}
    \end{center}
\end{figure}

==> Tables/autogluon_search_space.tex <==
\begin{table}[ht]
\begin{center}
%\footnotesize
%\begin{adjustbox}{width=\textwidth}{
\begin{tabular}{@{}lc@{}}
 \toprule
 \textbf{Parameter} & \textbf{Values} \\
 \midrule
  $Preset$ & 'Best Quality' \\ \midrule
 $Models$ & $\{\text{"FastAI"}, \text{"NN"}\}$ \\ \bottomrule
 \end{tabular}
%}\end{adjustbox}
\end{center}
\caption{\label{app:autogluon_search_space} The search space of the training parameters for AutoGluon.}
\end{table}

==> Tables/autosklearn_gb_config_space.tex <==
\begin{table}[ht!]
\centering
\footnotesize
\begin{adjustbox}{width=0.7\textwidth}{
\begin{tabular}{cc}
\toprule
 Argument & Value \\ \midrule
 \text{include\_estimator} & \{'gradient\_boosting'\} \\ \midrule
 \text{include\_preprocessors} & \{'no\_preprocessing'\} \\ \midrule
 \text{time\_left\_for\_this\_task} & \{'task dependent time'\} \\ \midrule
 \text{ensemble\_size} & \{1\} \\ \midrule
 \text{seed} & \{11\} \\ \midrule
 \text{memory\_limit} & \{6000\} \\ \midrule
 \text{initial\_configurations\_via\_metalearning} & \{0\} \\ \midrule
 \text{metric} & \{'balanced\_accuracy'\} \\ \midrule
  \text{n\_jobs} & \{10\} \\
\bottomrule
\end{tabular}}\end{adjustbox}
\caption{\textbf{Configuration for Auto-Sklearn.} The configuration used for Auto-Sklearn in the comparison with the Regularization Cocktail.}
\label{app:autosklearn_config_space}
\end{table}


==> Tables/cocktail_regularizers.tex <==
\begin{wraptable}[20]{r}{0.5\textwidth}
\centering
\footnotesize
\begin{tabular}{@{}lll@{}}
 \toprule
  \textbf{Group} & \textbf{Regularizer} & \textbf{Hyperparam}  \\
 \midrule
 \multirow{3}{*}{Implicit} & Batch Normalization &  $-$ \\ 
 & \multirow{2}{*}{Lookahead-Optimizer}  & 
 Step size \\
 & & Num. steps \\
 & SWA & - \\ \cmidrule{2-3}
 W. Decay &  Weight Decay & Decay factor \\
 \cmidrule{2-3}
 \multirow{2}{*}{M. Averaging} & \multirow{2}{*}{Drop-out}  & Dropout shape \\
 & & Drop rate \\
  & Snapshot Ensembles & Num. models \\  \cmidrule{2-3}
 \multirow{3}{*}{Structural} & Skip Connection & - \\
  & Shake-Shake & - \\ 
  & Shake-Drop & Max. probab.\\ \cmidrule{2-3}
 \multirow{4}{*}{Augment.} & Mix-Up & Magnitude \\ 
  & Cut-Mix & Probability \\ 
  & \multirow{2}{*}{Cut-Out}  & Probability \\
 & & Patch ratio \\ 
  & Adversarial & - \\
\bottomrule
\end{tabular}
\caption{\label{table:regularizer_hps} The cocktail regularizers and their corresponding hyperparameters.}
% For the regularization techniques, we will use the following abbrevations for the rest of the paper: (Batch Normalization: BN, Weight Decay: WD, Drop-Out: DO, Skip Connection: SC, Shake-Shake: SS, Shake-Drop: SD, Lookahead Optimizer: LA, Stochastic Weight Averaging: SWA, Snapshot Ensembles: SE, Mix-Up: MU, Cut-Mix: CM, Cut-Out: CO, and FGSM Adversarial Learning: AT)}
\vspace{-1.0cm}
\end{wraptable}

==> Tables/cocktail_vs_gbdt.tex <==
\begin{table*}[h]
\centering
\footnotesize
\begin{adjustbox}{width=1.0\textwidth}{
\begin{tabular}{lcclcclcclcclcc}
\toprule
{Task Id} & GBDT &  Cockt. & {Task Id} & GBDT &  Cockt. & {Task Id} & GBDT &  Cockt. & {Task Id} & GBDT &  Cockt.\\
\midrule
233090 &   90.000 &   89.270 &
233091 &   99.850 &   99.850 &
233092 &   46.850 &   61.461 &
233093 &   97.500 &   98.000 \\
233088 &   71.191 &   74.643 &
233094 &   80.165 &   82.576 &
233096 &   63.353 &   74.381 &
233099 &   79.830 &   82.443 \\
233102 &   62.764 &   63.923 &
233103 &   88.341 &   86.619 &
233104 &   99.967 &   99.953 &
233106 &   68.947 &   68.107 \\
233107 &   97.217 &   96.826 &
233108 &   93.519 &   95.833 &
233109 &   64.985 &   67.617 &
233110 &   72.283 &   85.993 \\
233112 &   72.645 &   80.073 &
233113 &   98.571 &   99.948 &
233114 &   72.926 &   73.546 &
233115 &   88.589 &   87.088 \\
233116 &  100.000 &   99.587 &
233117 &   93.074 &   93.723 &
233118 &   90.457 &   91.950 &
233119 &   83.070 &   97.471 \\
233120 &   52.421 &   52.668 &
233121 &   77.897 &   98.370 &
233122 & 21.144 & 27.70 & 
233123 &   55.593 &   65.287 \\
233124 &   63.428 &   71.667 &
233126 &   94.137 &   94.015 &
233130 &   91.797 &   92.535 &
233131 &   74.447 &   74.262 \\
233132 &   98.704 &   99.049 &
233133 &   70.120 &   69.183 &
233134 &   78.878 &   79.217 &
233135 &   95.119 &   94.045 \\
233137 & 74.620 & 94.01 &
233142 & 13.534 & 97.17 &
233143 &   92.514 &   92.531 &
233146 &   58.201 &   64.280 \\ 

\bottomrule
\end{tabular}} 
\end{adjustbox}
\caption{\textbf{Results of Experiment 3} The performances of the Regularization Cocktail and the GBDT algorithm over the different datasets.}
\label{app:cocktail_vs_gb_table}
\end{table*}


==> Tables/node_search_space.tex <==
\begin{table}[ht]
\begin{center}
%\footnotesize
%\begin{adjustbox}{width=\textwidth}{
\begin{tabular}{@{}llc@{}}
 \toprule
 \textbf{Hyperparameter} & \textbf{Type} & \textbf{Values} \\
 \midrule
  $num\_layers$ & Integer & $\{2\}$ \\ \midrule
 $total\_tree\_count$ & Integer & $\{1024\}$ \\ \midrule
 $tree\_depth$ & Integer & $\{6\}$ \\ \bottomrule 
\end{tabular}
%}\end{adjustbox}
\end{center}
\caption{\label{app:node_search_space} The search space of the training and model hyperparameters for NODE.}
\end{table}

==> Text/old_1_introduction.tex <==
\section{Introduction}

In most supervised learning application domains, the available data for training predictive models is both limited and noisy with respect to the target variable. Therefore, it is paramount to regularize machine learning models for generalizing the predictive performance on future unseen data. The concept of regularization is well-studied and constitutes one of the pillar components of machine learning. Throughout this work we use the term ``regularization'' for all methods that explicitly or implicitly take measures that reduce the overfitting phenomenon; we categorize these non-exhaustively into weight decay, data augmentation, model averaging, structure and linearization, and implicit regularization families (detailed in Section~\ref{sec:relatedwork}). In this paper, we propose a new principled strategy that highlights the need for automatically learning the optimal combination of regularizers, denoted as \textit{regularization cocktails}, via standard hyperparameter optimization.

%Truth be told, combining regularization methods is far from being a novel practice per se. As a matter of fact, most modern deep learning models use combinations of a number of regularizers. For instance, EfficientNet~\citep{pmlr-v97-tan19a} mixes components of structural regularization and linearization via ResNet-style skip connections~\citep{7780459}, learning rate scheduling, Drop-Out ensembling~\citep{10.5555/2627435.2670313} and AutoAugment data augmentation~\citep{Cubuk_2019_CVPR}. However, even though each of those regularizers is motivated in isolation, the reasoning behind a specific combination of regularizers is largely based on accuracy-driven manual trial-and-error iterations, mostly on image classification benchmarks like CIFAR~\citep{krizhevsky2009learning} and ImageNet~\citep{imagenet_cvpr09}. %It might not be entirely provocative to state that a large portion of the deep learning research in the last decade was spent on manually deriving both new and combined forms of regularization for neural networks. 

%Unfortunately, the manual search for combinations of regularizers is tedious, error-prone, unsustainable, and in essence constitutes an example of manual hyperparameter tuning, which in turn might be outperformed by automated algorithms~\citep{DBLP:conf/nips/SnoekLA12,thornton2013auto,10.5555/2969442.2969547,DBLP:conf/icml/OlsonM16,DBLP:conf/kdd/JinSH19,DBLP:journals/corr/abs-2003-06505,DBLP:journals/corr/abs-2006-13799}. 
%Following the spirit of AutoML~\citep{automl_book}, we, therefore propose a strategy for learning the optimal dataset-specific regularization cocktail by means of modern hyperparameter optimization (HPO). To the best of our knowledge, there exists no study providing empirical evidence that a mixture of numerous regularizers outperforms individual regularizers; this paper fills this gap. 
%%%More precisely, a research hypothesis of this paper is that a properly mixed regularization cocktail outperforms every individual regularizer in it, in terms of accuracy under the same run-time budget, and that the best cocktail to use depends on the dataset. To validate this hypothesis, we executed a large-scale experimental study employing 40 diverse tabular datasets and 13 prominent regularizers with thorough HPO for all regularizers. We focus on tabular datasets because, in contrast to large image datasets, thorough HPO is feasible. In addition, neural networks are high variance models for tabular datasets, therefore improved regularization schemes can provide a relatively higher generalization gain on tabular datasets compared to other data types. We further show that dataset-personalized regularization cocktails achieve state-of-the-art predictive accuracies on tabular data and significantly outperform strong baselines, such as XGBoost~\cite{Chen:2016:XST:2939672.2939785}.

In contrast to the mainstream in DL, in this paper we focus on tabular data, a domain that we feel is understudied in DL, yet of great relevance for many practical applications, such as climate science, medicine, manufacturing, finance, recommender systems, HR management, etc. While traditional machine learning methods, such as XGBoost~\cite{Chen:2016:XST:2939672.2939785}, dominate tabular data applications due to their superior performance compared to DL, extending the success story of DL to this domain would open up an extremely rich new set of applications for DL.

This paper is the first to provide compelling evidence that well-regularized DL methods 
indeed surpasses the current state of the art in tabular data sets, including XGBoost.
We believe this finding to potentially have far-reaching implications, and to open up a garden of delights of new applications for DL. 
%
Our individual contributions are as follows:

\begin{enumerate}
    \item We demonstrate that modern DL regularizers (developed for DL applications on raw data, such as images, speech, or text) also substantially improve the performance of DL methods on tabular data.
    \item We demonstrate the empirical accuracy gains of regularization cocktails over their individual ingredients in a systematic large-scale experimental study with 13 regularizers on 40 tabular datasets;
%    \item We challenge the status-quo practices of designing universal dataset-agnostic regularizers, by showing that an optimal regularization cocktail is highly dataset-dependent; \notefh{As far as I'm concerned, this is not very exciting and could be dropped as a contribution if push comes tho shove.}
    \item We demonstrate that regularization cocktails enable deep neural networks to outperform state-of-the-art prediction models for tabular data with a statistically-significant margin, outperforming XGBoost and thereby setting the new state-of-the-art in classifying tabular datasets;
     %\item We demonstrate that regularization cocktails achieve state-of-the-art classification accuracy performance on tabular datasets and outperform Gradient-Boosted Decision Trees (GBDT) with a statistically-significant margin;
    \item As an overarching contribution, we provide previously-lacking in-depth empirical evidence to better highlight the importance of combining different mechanisms for regularization, one of the most fundamental concepts in machine learning.
\end{enumerate}

%\notefh{Somehow, the intro still feels like some reviewers might get to here and still be in the mindset of ``this isn't surprising at all; why is this a paper?''. Of course, I disagree with that sentiment, but I'm having trouble putting into more exciting words why this is really important. So, what could we do to make this more ``exciting''? Off the top of my head, the only thing that comes to mind is to allude to the general importance of evidence-based research (rather than trusting folklore knowledge), and challenging readers to think of what work they would refer to for this folklore knowledge, or in teaching? Other ideas?}


%Although the outcomes of our research hypotheses might be perceived as intuitional and relatively well-known by some researchers, still, this paper is the first study to empirically confirm them.



==> Text/rebuttal_answer.tex <==
\begin{align}
\boldsymbol{\lambda}^* &\in \;  \argmin_{\boldsymbol{\lambda}^{(1)}, \dots,  \boldsymbol{\lambda}^{(K)}} \;\; \Ls\left(\mathbf{y}^{\text{(Val)}}, f\left(\mathbf{X}^{\text{(Val)}}; \boldsymbol{\theta}^{*}_{\boldsymbol{\lambda}} \right) \right)
\end{align}
